Expressive Reasoning Graph Store: A Unified Framework for Managing RDF and Property Graph Databases

Resource Description Framework (RDF) and Property Graph (PG) are the two most commonly used data models for representing, storing, and querying graph data. We present Expressive Reasoning Graph Store (ERGS) -- a graph store built on top of JanusGraph (a Property Graph store) that also allows storing and querying of RDF datasets. First, we describe how RDF data can be translated into a Property Graph representation and then describe a query translation module that converts SPARQL queries into a series of Gremlin traversals. The converters and translators thus developed can allow any Apache Tinkerpop compliant graph database to store and query RDF datasets. We demonstrate the effectiveness of our proposed approach using JanusGraph as the base Property Graph store and compare its performance with standard RDF systems.

==> figures/PropertyGraphBackground.tex <==
\section{Property Graphs Background}
\label{sec:graphBackground}
Property graph model has become popular in data storage, analytics, reasoning operation as it provides flexibility and efficiency in data storage and querying operations. Structurally, graphs store data in the form of nodes and edges, which helps in storing relationships physically. Nodes and edges also provide index free adjacency, i.e., in property graph model, presence of an edge between two vertices can be checked by visiting those vertices only without external indexing support. It makes running complex graph algorithms efficient such as connected component, page rank algorithms etc. Generally, real world problems are closely related to graphs that makes problem modeling easy into graph structure. Further, triple stores being strongly index based systems are good when relationship exploration is not very deep whereas graph databases are good at finding complex relations, and their compact representation helps in to speedup reasoning tasks by storing inferred information. 

Some well known property graphs, e.g. JanusGraph, facilitates to use different storage backend which can be setup distributively and helps in supporting data of huge size. Additionally, graphs also make use of popular indexing systems such as Elastic search and Solr for adding text related operation as part of graph query language.     

\subsection{Property Graph Data Model Description}
With the growth in popularity and application of graph databases there are many graph databases and graph database models available. We have picked Tinkerpop's Property graph model in our work given that it is very popular and widely adopted in various graph databases. 

We have used property graph model defined in~\cite{rod}. Consider property graph $G=(V,E,\lambda)$, where $V$ is set of vertices and $E$ is set of edges such that $E \subseteq (V \times V)$ and $\lambda : ((V \cup E) \times \Sigma^{\star}) \to (U \ 
\backslash \ (V \cup E))$ is partial function that maps string/element to object in universal set $U$ excluding vertices and edge. Given $\lambda$, vertices and edges can have arbitrary number of edges key/value pairs called properties. Tinkerpop based graphs also support meta properties which means a property can have properties that property of property.

==> files/OldSystemArchitecture1.tex <==
\section{System Architecture}
The high level architecture of the proposed system is describe in Figure~\ref{fig:SysArch} and we describe the different components in detail below.
\begin{figure}
	\centering
	\includegraphics[width=1\columnwidth]{figures/Architecture.png}
	\caption{System Architecture}
	\label{fig:SysArch}
\end{figure}
%\begin{itemize}


\noindent
{\bf Ingestion Module:} Ingestion module is responsible for ingesting data from end user and creating a knowledge base. Current ingestion module supports RDF/OWL/Text data as standard input data. We implemented all the standard RDF4J ingestion related APIs as part of this module to support RDF data ingestion. More details about the way RDF data is mapped to underlying storage model is described in the Section~\ref{sec:ingestion}. Ingestion module also supplies the knowledge base data along with the OWL data to create summary knowledge graph that is later used in the query processing.
Ingestion module also takes any text documents that are associated with the given knowledge base and computes context for each entity in the knowledge base to support some of the custom operations like entity resolution, context based node search kind of operations.

\noindent
{\bf Knowledge Layer:}
We chose JanusGraph (a property graph) as our default storage technology to store knowledge base along with additional metadata such as context, evidence etc. Since property graphs can easily capture the context/confidence etc in the form of node or edge properties, it becomes easier to map these information coming from the data curation pipelines easily at one place. During ingestion, user data in various commonly used formats is converted and stored in the back-end storage. In order to ingest OWL/RDF, data we have implemented RDF4J framework to add JanusGraph as additional store implementing data store interfaces. This takes RDF/OWL data in various forms and maps it to appropriate property graph model and creates required indices as well. We also store information like context for a given entity computed from the textual input data (if given) along with the knowledge base in the form of RDF/OWL data. This is mapped as an additional text property for each node corresponding to an entity int he JanusGraph node.
    
 \noindent
 {\bf Query Processing Module:} This Module is responsible for handling the user query requests coming in the form of SPARQL/custom API queries. 
 This module acts like a middleware layer between the specific processing modules like SPARQL to Gremlin, Summarization Module, Custom modules and the User APIs that are exposed to the end user. Bulk of the query routing, Query expansion and other complex reasoning query processing logic is embedded into this layer. 
 
 \noindent
 {\bf SPARQL-Gremlin Module:} This module is responsible for converting a given SPARQL query into an appropriate Gremlin traversal using the meta data that ingestion layer generates. More details about this module are described in the Section~\ref{sec:queryEngine}.
 
 \noindent
 {\bf Summerization Module:} This module is one of the key component for supporting reasoning on large ABox data. We use summary based query answering mechanism described in SHER system ~\cite{SHER}as key component for answering queries that require complex reasoning requirement. This module also hosts a in-memory reasoner to perform basic reasoning operations like consistency check, justification generation. In our system we used JFact~\cite{JFact} as a in memory reasoner to support these basic reasoning operations. We used standard OWLAPIs to interact with the in memory reasoner and hence this can be replaced with any compatible in-memory reasoner. There are two major operations that are performed by this module first one is summary generation and storage and the second one is summary based query answering. Summary of the given ABox data of a knowledge base is generated in such a way that if the summarized knowledge base is consistent then we can safely say that underlying full knowledge base is also consistent. More details about how this summary is generated and related theoretical results on these guarantees one can refer to ~\cite{SHER}. Generated summary is stored along with the knowledge base in the form of graph with connections to appropriate individuals in the JanusGraph. Please note that original SHER work is based on DB2 back-end and we implemented these modules on top of property graph framework to work with JanusGraph. Second main task of this module is to support query processing for queries involving knowledge bases with complex reasoning requirements. We use the summary based refinement technique described in the SHER system to iteratively refine the summary to answer a query using the basic reaoning operations supported by an in-memory reasoner.
 
 \noindent
 {\bf Custom Modules:Sumit B to modify it further} This module is responsible for supporting additional non symbolic reasoning related operations. In the current system we have implemented context model based operations like, entity resolution, node search etc. These modules take plain text or keywords as input and output nodes as output based on the degree of match between nodes and context data stored for each node with the incoming textual data.
 
 \noindent
 {\bf API Layer:} This layer is the user facing layer which hosts all the APIs in the form of REST and JavaAPIs for a user to interact with the underlying system. It currently has all the RDF4J ingestion /querying APIs along with the context based APIs that are supported as part of custom operations supported.
 %. For queries involving reasoning, we use two approaches to handle the queries depending the expressivity of the underlying Knowledge base. For OWL Profiles that are below OWL-QL expressivity we use query translation described in ~\cite{quartzel} system to expand the given user query to account for required reasoning. For the OWL profiles requiring more complex reasoning we use summery based query evaluation technique described in ~\cite{SHER} system.
 
 
%\comment{For the queries requiring reasoning it talks to the underlying reasoner to get the answers. For example in case of symbolic reasoner, this unit will talk to symbolic reasoner using OWL APIs to get the TBox  inference to do the query expansion or query rewrite. In cases where complex reasoning is needed, it sends the required ABox summary information to the reasoner to generate the answer. We are planning to implement the ABox summary builder described in the SHER system\cite{SHER} to work with JanusGraph backend.  We have extended RDF4J query interfaces for basic RDF querying.}
    
 \noindent
 %{\bf Reasoners:} This component is responsible for standing up different reasoners with appropriate APIs to talk to the query and storage layers. In the current implementation, we are integrating Racer\cite{racer} using OWL APIs to support TBox reasoning and also plays a role in query answering using SHER system. We will be extending this to include neural reasoner and default IR/Text reasoner to get a search answer in scenarios where we don't get confident answers from other reasoners. 
%\end{itemize}


==> files/backend-storage.tex <==
\section{Graph Database for Reasoning}
The choice of storage technology is crucial for efficient implementation of underlying reasoning engines. While the in-memory reasoners maintain complete ABox data in memory leading to quick query times, systems designed for dealing large ABoxes store data in persistent storage backends such as relational database or triple stores. At query time, the required data is fetched and passed on to the reasoner for inference.% There exists many reasoners which are based on relational backend such as SHER~\cite{SHER}, OnTop~\cite{Ontop13}, alternatively, Triple stores is used in Virtuoso\footnote{https://virtuoso.openlinksw.com}. 

We adopt a property graph database as our persistent ABox store. Graph databases have become quite popular for data storage due to their flexible schema and close relation of the storage model with real-world data. Such graph databases store data in the form of nodes and edges, provide index-free adjacency, and therefore, perform  potentially better on linked datasets. Compared to relational databases, graph databases are better at join intensive queries~\cite{Vicknair10}. Further, triple stores being strongly index based systems are good when relationship exploration is not very deep whereas graph databases are good at finding complex relations, and their compact representation helps in to speedup reasoning tasks by storing inferred information.%With the ability of modeling relationships, graph database can be helpful in complex reasoning operations. Moreover, with compact representation, compare to Triple store, graph database are useful in storing inferred information to speedup reasoning tasks.



==> files/notes.tex <==
\section{Notes}

Notes for experiments:
\begin{enumerate}
    \item We can use SP2 benchmark or LUBM benchmark to test the performance
    \item We can also use the SPARQL test cases
    \item BSBM has 12 queries
    \item Ingestion: We have not done any kind of graph analysis on this. That could also be done. We could have an argument that translation could also help in graph based operations. Report number of edges and nodes in the graph, Adamic Adar and Page Rank can also be done. We can have a small section on graph based methods also.
    \item Gremlinator needs to convert RDF to PG also.
    \item Stores: Virtuoso, Blazegraph, Ergo, Ergo with Gremlinator (forward chaining)
    \item Datasets: SP2, BSBM, LUBM 
    \item 
\end{enumerate}
